Small subgraphs in the trace of a random walk

We consider the combinatorial properties of the trace of a random walk on the complete graph and on the random graph $G(n,p)$. In particular, we study the appearance of a fixed subgraph in the trace. We prove that for a subgraph containing a cycle, the threshold for its appearance in the trace of a random walk of length $m$ is essentially equal to the threshold for its appearance in the random graph drawn from $G(n,m)$. In the case where the base graph is the complete graph, we show that a fixed forest appears in the trace typically much earlier than it appears in $G(n,m)$.

==> commands.tex <==
\usepackage{bbm}

\usepackage{mleftright}
\mleftright
\usepackage{amsmath,amssymb}

\newcommand\numberthis{\addtocounter{equation}{1}\tag{\theequation}}

%%%%% Flexible operators %%%%%
\makeatletter
%% Expectation %%
\newcommand*{\E}{%
  \def\E@sub{}%
  \def\E@sup{}%
  \E@scripts
}
\newcommand*{\E@scripts}{%
  \@ifnextchar_\E@subscript{%
    \@ifnextchar^\E@supscript\E@finish
  }%
}
\def\E@subscript_#1{%
  \ifx\E@sub\@empty
    \def\E@sub{#1}%
  \else
    \errmessage{E already has a subscript}%
  \fi
  \E@scripts
}
\def\E@supscript^#1{%
  \ifx\E@sup\@empty
    \def\E@sup{#1}%
  \else
    \errmessage{E already has a superscript}%
  \fi
  \E@scripts
}
\newcommand*{\E@finish}[1]{%
  \mathbb{E}%
  \ifx\E@sub\@empty\else _{\E@sub}\fi
  \ifx\E@sup\@empty\else ^{\E@sup}\fi
  \left(#1\right)%
}

%% Probability %%
\newcommand*{\pr}{%
  \def\pr@sub{}%
  \def\pr@sup{}%
  \pr@scripts
}
\newcommand*{\pr@scripts}{%
  \@ifnextchar_\pr@subscript{%
    \@ifnextchar^\pr@supscript\pr@finish
  }%
}
\def\pr@subscript_#1{%
  \ifx\pr@sub\@empty
    \def\pr@sub{#1}%
  \else
    \errmessage{E already has a subscript}%
  \fi
  \pr@scripts
}
\def\pr@supscript^#1{%
  \ifx\pr@sup\@empty
    \def\pr@sup{#1}%
  \else
    \errmessage{E already has a superscript}%
  \fi
  \pr@scripts
}
\newcommand*{\pr@finish}[1]{%
  \mathbb{P}%
  \ifx\pr@sub\@empty\else _{\pr@sub}\fi
  \ifx\pr@sup\@empty\else ^{\pr@sup}\fi
  \left(#1\right)%
}
\makeatother


\newcommand{\midd}[0]{\ \big\vert\ }

%%%%% Functions %%%%%
\newcommand{\lln}[1]{\ln{\ln{#1}}}
\newcommand{\llln}[1]{\ln\ln\ln{#1}}
\newcommand{\floor}[1]{\left\lfloor{#1}\right\rfloor}
\newcommand{\ceil}[1]{\left\lceil{#1}\right\rceil}
\renewcommand{\exp}[1]{\text{exp}\left(#1\right)}
%\DeclareMathOperator{\exp}{exp}
\newcommand{\I}[1]{\mathbbm{1}_{#1}}

%%%%% Set Theory %%%%%
%% Indicator
\newcommand{\ind}[2]{\mathbbm{1}_{#1}\left({#2}\right)}
%% Disjoint union
\makeatletter
\def\moverlay{\mathpalette\mov@rlay}
\def\mov@rlay#1#2{\leavevmode\vtop{%
   \baselineskip\z@skip \lineskiplimit-\maxdimen
   \ialign{\hfil$\m@th#1##$\hfil\cr#2\crcr}}}
\newcommand{\charfusion}[3][\mathord]{
    #1{\ifx#1\mathop\vphantom{#2}\fi
        \mathpalette\mov@rlay{#2\cr#3}
      }
    \ifx#1\mathop\expandafter\displaylimits\fi}
\makeatother

\newcommand{\cupdot}{\charfusion[\mathbin]{\cup}{\cdot}}
\newcommand{\bigcupdot}{\charfusion[\mathop]{\bigcup}{\cdot}}

%% Important sets
\newcommand{\NN}[0]{\mathbb{N}}
\newcommand{\ZZ}[0]{\mathbb{Z}}
\newcommand{\QQ}[0]{\mathbb{Q}}
\newcommand{\RR}[0]{\mathbb{R}}
\newcommand{\CC}[0]{\mathbb{C}}

%%%%% Probability %%%%%
\newcommand{\var}[1]{\text{Var}\left(#1\right)}
\DeclareMathOperator{\cov}{Cov}
%\newcommand{\cov}[2]{\text{Cov}\left(#1,#2\right)}

%% Distributions
\newcommand{\ber}[1]{\text{Bernoulli}\left(#1\right)}
\newcommand{\bin}[2]{\text{Bin}\left(#1,#2\right)}
\newcommand{\geom}[1]{\text{Geom}\left(#1\right)}
\newcommand{\hypg}[3]{\text{Hypergeometric}\left(#1,#2,#3\right)}
\newcommand{\unif}[1]{\text{Uniform}\left(#1\right)}

%% Misc.
\newcommand{\iid}[0]{\textbf{i.i.d.}\ }
\newcommand{\whp}[0]{\textbf{whp}}
\newcommand{\dtv}[2]{d_{TV}(#1,#2)}

%%%%% Linear Algebra %%%%%
%% Diag
\newcommand{\diag}[1]{\text{diag}\left(#1\right)}

%% Rank
\newcommand{\rank}[1]{\text{rank}\left(#1\right)}

%% Permutation
\newcommand{\perm}[1]{\text{perm}\left(#1\right)}

%% Span
% This command is offending (clashing with \align)
%\renewcommand{\span}[1]{\text{span}#1}

%% Trace
\newcommand{\tr}[1]{\text{tr}\left(#1\right)}

%% Vectors
\newcommand{\vc}[1]{\mathbf{#1}}
\newcommand{\one}[0]{\v{1}}

%% Special set names
\newcommand{\End}[1]{\text{End}\left({#1}\right)}
\newcommand{\fit}[1]{\text{FIT}\left(#1\right)}
%\newcommand{\Small}[0]{\text{SMALL}}

%%%%% Graph Theory %%%%%
%% Random graphs
\newcommand{\gdrn}[0]{G(d,r,n)}
\newcommand{\gmn}[0]{G(m,n)}
\newcommand{\gnm}[0]{G(n,m)}
\newcommand{\gnp}[0]{G(n,p)}
\newcommand{\dnp}[0]{D(n,p)}
\newcommand{\gnr}[0]{G(n,r)}
\newcommand{\gp}[0]{G_p}

%% Misc.
% Circumference
\DeclareMathOperator{\Cir}{cir}
% Crossing number
\DeclareMathOperator{\Cr}{cr}
% Number of odd vertices
\DeclareMathOperator{\odd}{odd}

%%%%% Probability %%%%%
%% Convergence
\newcommand{\asto}[0]{\xrightarrow{a.s.}}
\newcommand{\downto}[0]{\searrow}
\newcommand{\upto}[0]{\nearrow}

%%%%% Mathematicians %%%%%
\newcommand{\bollobas}[0]{{Bollob\'as}}
\newcommand{\cerny}[0]{{{\v{C}}ern{\'y}}}
\newcommand{\chvatal}[0]{{Chv{\'a}tal}}
\newcommand{\erdos}[0]{{Erd\H{o}s}}
\newcommand{\komlos}[0]{{Koml\'os}}
\newcommand{\lovasz}[0]{{Lov{\'a}sz}}
\newcommand{\luczak}[0]{{\L uczak}}
\newcommand{\posa}[0]{{P\'{o}sa}}
\newcommand{\renyi}[0]{{R\'enyi}}
\newcommand{\rucinski}[0]{{Ruci{\'n}ski}}
\newcommand{\szemeredi}[0]{{Szemer\'edi}}

%%%%% Other %%%%%
\newcommand{\diam}[1]{\text{diam}\left(#1\right)}
\newcommand{\erf}[1]{\text{erf}\left(#1\right)}

%%%%% Notes %%%%%
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\blue}[1]{{\color{blue}#1}}
\newcommand{\green}[1]{{\color{green}#1}}
%\newcommand{\todo}[0]{{\bf\red{TODO:}} }
\newcommand{\tba}[1]{{\bf\red{TBA}} --- #1}

%% Positional Games %%
\newcommand{\Red}[0]{{\red{Red}}}
\newcommand{\Blue}[0]{{\blue{Blue}}}

%% Random Walks %%
\DeclareMathOperator{\hit}{hit}
\DeclareMathOperator{\rng}{rng}
\DeclareMathOperator{\trace}{trace}
\newcommand{\tmix}{t_{\mathrm{mix}}}


